Structural Ramsey theory of metric spaces and topological dynamics of isometry groups

In 2003, Kechris, Pestov and Todorcevic showed that the structure of certain separable metric spaces - called ultrahomogeneous - is closely related to the combinatorial behavior of the class of their finite metric spaces. The purpose of the present paper is to explore the different aspects of this connection.

==> Notations2.tex <==
%\documentclass{amsbook}
%\usepackage{amsmath,amsfonts,amssymb,amsthm,enumerate,latexsym,mathrsfs,lineno}
%\usepackage[dvips]{graphicx}
%\usepackage[latin1]{inputenc}
%\usepackage[francais]{babel}
%\input{Macros}

%\begin{document}

\chapter*{Preliminary remarks.}

The notations which are used in the present thesis are fairly standard. Nevertheless, a choice was sometimes needed. In particular: 

Open intervals of real numbers are written according to the French convention. For example, for $a < b \in \R \cup \{ - \infty \} \cup \{ + \infty \}$, $\{ x \in \R : a < x < b \}$ is written $]a,b[$\index{$]a,b[$}.

Set-theoretic inclusion is also written according to the French convention, that is $\subset$\index{$\subset$, $\subsetneq$}, while strict inclusion is written $\subsetneq$.  
 
A natural number is often seen as the set of its strict predecessors. In particular, $k = \{0, 1,\ldots , k-1 \}$ whenever $k > 0$. On the other hand, the set of all natural numbers is written according to the ordinal convention, that is $\omega$\index{$\omega$}. 

Given a set $X$, its cardinality is written $\left| X \right|$\index{$\left| X \right|$}. 

Given sets $X_0 \subset X$, $Y_0 \subset Y$ and a function $f : \funct{X}{Y}$, the direct image of $X_0$ by $f$ is written $f''X_0$\index{$f''X_0$, $\overleftarrow{f}Y_0$, $\restrict{f}{X_0}$} and the inverse image of $Y_0$ by $f$ is written $\overleftarrow{f}Y_0$. The restriction of $f$ to $X_0$ is written $\restrict{f}{X_0}$. When $f$ is specified without $X$ and $Y$, $\dom f$\index{$\dom f$} refers to its domain and $\ran f$\index{$\ran f$} to its range. 

Finally, if $\prec$ is a linear ordering on a set $X$ and $x, y \in X$, then $\{ x, y \}_{\prec}$\index{$\{ x, y \}_{\prec}$, $\{ s_i : i \in \omega\}_{\prec}$} represents the set $\{ x, y \}$ being understood that $x \prec y$. Similarly, $\{ s_i : i \in \omega\}_{\prec}$ denotes the set $\{ s_i : i \in \omega\}$, being understood that $s_i \prec s_j$ whenever $i<j$.




%\end{document}   
